Average treatment effects in the presence of unknown interference

We investigate large-sample properties of treatment effect estimators under unknown interference in randomized experiments. The inferential target is a generalization of the average treatment effect estimand that marginalizes over potential spillover effects. We show that estimators commonly used to estimate treatment effects under no interference are consistent for the generalized estimand for several common experimental designs under limited but otherwise arbitrary and unknown interference. The rates of convergence depend on the rate at which the amount of interference grows and the degree to which it aligns with dependencies in treatment assignment. Importantly for practitioners, the results imply that if one erroneously assumes that units do not interfere in a setting with limited, or even moderate, interference, standard estimators are nevertheless likely to be close to an average treatment effect if the sample is sufficiently large. Conventional confidence statements may, however, not be accurate.

==> tab-groupsum-bias.tex <==
\begin{tabular}{l p{0.1in} rrrr p{0.15in} rrrr}
\multicolumn{11}{l}{Panel A: Bernoulli randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.006 & 0.005 & 0.000 & 0.000 &  & 0.002 & 0.000 & 0.000 & 0.000 \\
$25$ &  & 0.011 & 0.000 & 0.000 & 0.000 &  & 0.035 & 0.005 & 0.000 & 0.000 \\
$8 n^{0.25}$ &  & 0.011 & 0.001 & 0.000 & 0.000 &  & 0.035 & 0.005 & 0.001 & 0.000 \\
$2.5 n^{0.5}$ &  & 0.011 & 0.000 & 0.000 & 0.001 &  & 0.035 & 0.007 & 0.001 & 0.001 \\
$0.25n$ &  & 0.011 & 0.002 & 0.000 & 0.004 &  & 0.035 & 0.011 & 0.004 & 0.005 \\
$n$ &  & 0.014 & 0.014 & 0.005 & 0.001 &  & 0.074 & 0.035 & 0.003 & 0.004 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel B: Complete randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.003 & 0.000 & 0.000 & 0.000 &  & 0.003 & 0.000 & 0.000 & 0.000 \\
$25$ &  & 0.041 & 0.004 & 0.000 & 0.000 &  & 0.041 & 0.004 & 0.000 & 0.000 \\
$8 n^{0.25}$ &  & 0.041 & 0.006 & 0.000 & 0.000 &  & 0.041 & 0.006 & 0.000 & 0.000 \\
$2.5 n^{0.5}$ &  & 0.041 & 0.009 & 0.001 & 0.000 &  & 0.041 & 0.009 & 0.001 & 0.000 \\
$0.25n$ &  & 0.041 & 0.015 & 0.005 & 0.001 &  & 0.041 & 0.015 & 0.005 & 0.001 \\
$n$ &  & 0.997 & 1.000 & 1.000 & 1.000 &  & 0.997 & 1.000 & 1.000 & 1.000 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel C: Paired randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.001 & 0.000 & 0.000 & 0.000 &  & 0.001 & 0.000 & 0.000 & 0.000 \\
$25$ &  & 0.047 & 0.004 & 0.000 & 0.000 &  & 0.047 & 0.004 & 0.000 & 0.000 \\
$8 n^{0.25}$ &  & 0.047 & 0.006 & 0.001 & 0.000 &  & 0.047 & 0.006 & 0.001 & 0.000 \\
$2.5 n^{0.5}$ &  & 0.047 & 0.006 & 0.002 & 0.001 &  & 0.047 & 0.006 & 0.002 & 0.001 \\
$0.25n$ &  & 0.047 & 0.014 & 0.007 & 0.003 &  & 0.047 & 0.014 & 0.007 & 0.003 \\
$n$ &  & 0.999 & 1.000 & 1.000 & 1.000 &  & 0.999 & 1.000 & 1.000 & 1.000 \\
\bottomrule \multicolumn{11}{l}{\footnotesize Note: Each cell presents the result from 50,000 draws from the data generating process.} \\
\end{tabular}


==> tab-groupsum-sd.tex <==
\begin{tabular}{l p{0.1in} rrrr p{0.15in} rrrr}
\multicolumn{11}{l}{Panel A: Bernoulli randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 1.181 & 0.375 & 0.119 & 0.037 &  & 0.444 & 0.139 & 0.044 & 0.014 \\
$25$ &  & 1.571 & 0.500 & 0.157 & 0.050 &  & 0.645 & 0.204 & 0.064 & 0.020 \\
$8 n^{0.25}$ &  & 1.571 & 0.546 & 0.194 & 0.070 &  & 0.645 & 0.245 & 0.100 & 0.040 \\
$2.5 n^{0.5}$ &  & 1.571 & 0.607 & 0.259 & 0.119 &  & 0.645 & 0.303 & 0.165 & 0.090 \\
$0.25n$ &  & 1.571 & 0.822 & 0.595 & 0.530 &  & 0.645 & 0.523 & 0.504 & 0.502 \\
$n$ &  & 2.037 & 1.302 & 1.091 & 1.028 &  & 1.088 & 1.010 & 1.001 & 1.000 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel B: Complete randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.440 & 0.139 & 0.044 & 0.014 &  & 0.440 & 0.139 & 0.044 & 0.014 \\
$25$ &  & 0.510 & 0.163 & 0.051 & 0.016 &  & 0.510 & 0.163 & 0.051 & 0.016 \\
$8 n^{0.25}$ &  & 0.510 & 0.180 & 0.070 & 0.027 &  & 0.510 & 0.180 & 0.070 & 0.027 \\
$2.5 n^{0.5}$ &  & 0.510 & 0.207 & 0.106 & 0.054 &  & 0.510 & 0.207 & 0.106 & 0.054 \\
$0.25n$ &  & 0.510 & 0.331 & 0.301 & 0.298 &  & 0.510 & 0.331 & 0.301 & 0.298 \\
$n$ &  & 0.440 & 0.139 & 0.044 & 0.014 &  & 0.440 & 0.139 & 0.044 & 0.014 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel C: Paired randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.404 & 0.127 & 0.040 & 0.013 &  & 0.404 & 0.127 & 0.040 & 0.013 \\
$25$ &  & 0.477 & 0.151 & 0.048 & 0.015 &  & 0.477 & 0.151 & 0.048 & 0.015 \\
$8 n^{0.25}$ &  & 0.477 & 0.171 & 0.068 & 0.026 &  & 0.477 & 0.171 & 0.068 & 0.026 \\
$2.5 n^{0.5}$ &  & 0.477 & 0.198 & 0.104 & 0.054 &  & 0.477 & 0.198 & 0.104 & 0.054 \\
$0.25n$ &  & 0.477 & 0.324 & 0.299 & 0.297 &  & 0.477 & 0.324 & 0.299 & 0.297 \\
$n$ &  & 0.404 & 0.127 & 0.040 & 0.013 &  & 0.404 & 0.127 & 0.040 & 0.013 \\
\bottomrule \multicolumn{11}{l}{\footnotesize Note: Each cell presents the result from 50,000 draws from the data generating process.} \\
\end{tabular}


==> tab-oneunit-bias.tex <==
\begin{tabular}{l p{0.1in} rrrr p{0.15in} rrrr}
\multicolumn{11}{l}{Panel A: Bernoulli randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.006 & 0.005 & 0.000 & 0.000 &  & 0.002 & 0.000 & 0.000 & 0.000 \\
$24^{0.5}n^{0.5}$ &  & 0.008 & 0.006 & 0.000 & 0.000 &  & 0.005 & 0.001 & 0.000 & 0.000 \\
$8^{0.5}n^{0.625}$ &  & 0.008 & 0.006 & 0.000 & 0.000 &  & 0.005 & 0.002 & 0.001 & 0.000 \\
$2.5^{0.5}n^{0.75}$ &  & 0.008 & 0.007 & 0.001 & 0.001 &  & 0.005 & 0.002 & 0.001 & 0.001 \\
$0.5n$ &  & 0.008 & 0.008 & 0.003 & 0.003 &  & 0.005 & 0.004 & 0.004 & 0.003 \\
$n$ &  & 0.010 & 0.012 & 0.007 & 0.007 &  & 0.009 & 0.008 & 0.007 & 0.007 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel B: Complete randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.003 & 0.000 & 0.000 & 0.000 &  & 0.003 & 0.000 & 0.000 & 0.000 \\
$24^{0.5}n^{0.5}$ &  & 0.001 & 0.001 & 0.000 & 0.000 &  & 0.001 & 0.001 & 0.000 & 0.000 \\
$8^{0.5}n^{0.625}$ &  & 0.001 & 0.001 & 0.001 & 0.000 &  & 0.001 & 0.001 & 0.001 & 0.000 \\
$2.5^{0.5}n^{0.75}$ &  & 0.001 & 0.002 & 0.001 & 0.000 &  & 0.001 & 0.002 & 0.001 & 0.000 \\
$0.5n$ &  & 0.001 & 0.004 & 0.004 & 0.003 &  & 0.001 & 0.004 & 0.004 & 0.003 \\
$n$ &  & 0.004 & 0.008 & 0.007 & 0.006 &  & 0.004 & 0.008 & 0.007 & 0.006 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel C: Paired randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.001 & 0.000 & 0.000 & 0.000 &  & 0.001 & 0.000 & 0.000 & 0.000 \\
$24^{0.5}n^{0.5}$ &  & 0.006 & 0.002 & 0.001 & 0.000 &  & 0.006 & 0.002 & 0.001 & 0.000 \\
$8^{0.5}n^{0.625}$ &  & 0.006 & 0.003 & 0.001 & 0.000 &  & 0.006 & 0.003 & 0.001 & 0.000 \\
$2.5^{0.5}n^{0.75}$ &  & 0.006 & 0.004 & 0.001 & 0.001 &  & 0.006 & 0.004 & 0.001 & 0.001 \\
$0.5n$ &  & 0.006 & 0.007 & 0.002 & 0.004 &  & 0.006 & 0.007 & 0.002 & 0.004 \\
$n$ &  & 0.013 & 0.014 & 0.004 & 0.007 &  & 0.013 & 0.014 & 0.004 & 0.007 \\
\bottomrule \multicolumn{11}{l}{\footnotesize Note: Each cell presents the result from 50,000 draws from the data generating process.} \\
\end{tabular}


==> tab-oneunit-sd.tex <==
\begin{tabular}{l p{0.1in} rrrr p{0.15in} rrrr}
\multicolumn{11}{l}{Panel A: Bernoulli randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 1.181 & 0.375 & 0.119 & 0.037 &  & 0.444 & 0.139 & 0.044 & 0.014 \\
$24^{0.5}n^{0.5}$ &  & 1.316 & 0.409 & 0.129 & 0.041 &  & 0.650 & 0.206 & 0.066 & 0.021 \\
$8^{0.5}n^{0.625}$ &  & 1.326 & 0.436 & 0.150 & 0.053 &  & 0.665 & 0.252 & 0.100 & 0.040 \\
$2.5^{0.5}n^{0.75}$ &  & 1.326 & 0.475 & 0.199 & 0.096 &  & 0.665 & 0.312 & 0.164 & 0.090 \\
$0.5n$ &  & 1.326 & 0.634 & 0.515 & 0.501 &  & 0.665 & 0.517 & 0.502 & 0.500 \\
$n$ &  & 1.619 & 1.078 & 1.008 & 1.001 &  & 1.087 & 1.008 & 1.001 & 1.000 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel B: Complete randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.440 & 0.139 & 0.044 & 0.014 &  & 0.440 & 0.139 & 0.044 & 0.014 \\
$24^{0.5}n^{0.5}$ &  & 0.646 & 0.206 & 0.066 & 0.021 &  & 0.646 & 0.206 & 0.066 & 0.021 \\
$8^{0.5}n^{0.625}$ &  & 0.661 & 0.252 & 0.100 & 0.040 &  & 0.661 & 0.252 & 0.100 & 0.040 \\
$2.5^{0.5}n^{0.75}$ &  & 0.661 & 0.312 & 0.164 & 0.090 &  & 0.661 & 0.312 & 0.164 & 0.090 \\
$0.5n$ &  & 0.661 & 0.517 & 0.502 & 0.500 &  & 0.661 & 0.517 & 0.502 & 0.500 \\
$n$ &  & 1.083 & 1.007 & 1.001 & 1.000 &  & 1.083 & 1.007 & 1.001 & 1.000 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel C: Paired randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.404 & 0.127 & 0.040 & 0.013 &  & 0.404 & 0.127 & 0.040 & 0.013 \\
$24^{0.5}n^{0.5}$ &  & 0.623 & 0.200 & 0.063 & 0.020 &  & 0.623 & 0.200 & 0.063 & 0.020 \\
$8^{0.5}n^{0.625}$ &  & 0.638 & 0.247 & 0.098 & 0.040 &  & 0.638 & 0.247 & 0.098 & 0.040 \\
$2.5^{0.5}n^{0.75}$ &  & 0.638 & 0.308 & 0.163 & 0.090 &  & 0.638 & 0.308 & 0.163 & 0.090 \\
$0.5n$ &  & 0.638 & 0.516 & 0.502 & 0.500 &  & 0.638 & 0.516 & 0.502 & 0.500 \\
$n$ &  & 1.071 & 1.008 & 1.001 & 1.000 &  & 1.071 & 1.008 & 1.001 & 1.000 \\
\bottomrule \multicolumn{11}{l}{\footnotesize Note: Each cell presents the result from 50,000 draws from the data generating process.} \\
\end{tabular}


==> tab-random-bias.tex <==
\begin{tabular}{l p{0.1in} rrrr p{0.15in} rrrr}
\multicolumn{11}{l}{Panel A: Bernoulli randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.006 & 0.005 & 0.000 & 0.000 &  & 0.002 & 0.000 & 0.000 & 0.000 \\
$5$ &  & 0.002 & 0.001 & 0.000 & 0.000 &  & 0.014 & 0.002 & 0.000 & 0.000 \\
$8^{0.5}n^{0.125}$ &  & 0.006 & 0.002 & 0.001 & 0.000 &  & 0.016 & 0.001 & 0.000 & 0.000 \\
$2.5^{0.5}n^{0.25}$ &  & 0.002 & 0.001 & 0.001 & 0.000 &  & 0.014 & 0.003 & 0.000 & 0.000 \\
$0.05n$ &  & 0.002 & 0.002 & 0.001 & 0.000 &  & 0.014 & 0.006 & 0.002 & 0.000 \\
$n$ &  & 0.014 & 0.014 & 0.005 & 0.001 &  & 0.074 & 0.035 & 0.003 & 0.004 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel B: Complete randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.003 & 0.000 & 0.000 & 0.000 &  & 0.003 & 0.000 & 0.000 & 0.000 \\
$5$ &  & 0.014 & 0.002 & 0.000 & 0.000 &  & 0.014 & 0.002 & 0.000 & 0.000 \\
$8^{0.5}n^{0.125}$ &  & 0.016 & 0.002 & 0.000 & 0.000 &  & 0.016 & 0.002 & 0.000 & 0.000 \\
$2.5^{0.5}n^{0.25}$ &  & 0.014 & 0.002 & 0.000 & 0.000 &  & 0.014 & 0.002 & 0.000 & 0.000 \\
$0.05n$ &  & 0.014 & 0.006 & 0.002 & 0.001 &  & 0.014 & 0.006 & 0.002 & 0.001 \\
$n$ &  & 0.997 & 1.000 & 1.000 & 1.000 &  & 0.997 & 1.000 & 1.000 & 1.000 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel C: Paired randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.001 & 0.000 & 0.000 & 0.000 &  & 0.001 & 0.000 & 0.000 & 0.000 \\
$5$ &  & 0.015 & 0.001 & 0.000 & 0.000 &  & 0.015 & 0.001 & 0.000 & 0.000 \\
$8^{0.5}n^{0.125}$ &  & 0.015 & 0.002 & 0.000 & 0.000 &  & 0.015 & 0.002 & 0.000 & 0.000 \\
$2.5^{0.5}n^{0.25}$ &  & 0.015 & 0.002 & 0.000 & 0.000 &  & 0.015 & 0.002 & 0.000 & 0.000 \\
$0.05n$ &  & 0.015 & 0.006 & 0.001 & 0.001 &  & 0.015 & 0.006 & 0.001 & 0.001 \\
$n$ &  & 0.999 & 1.000 & 1.000 & 1.000 &  & 0.999 & 1.000 & 1.000 & 1.000 \\
\bottomrule \multicolumn{11}{l}{\footnotesize Note: Each cell presents the result from 50,000 draws from the data generating process.} \\
\end{tabular}


==> tab-random-sd.tex <==
\begin{tabular}{l p{0.1in} rrrr p{0.15in} rrrr}
\multicolumn{11}{l}{Panel A: Bernoulli randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 1.181 & 0.375 & 0.119 & 0.037 &  & 0.444 & 0.139 & 0.044 & 0.014 \\
$5$ &  & 1.337 & 0.422 & 0.133 & 0.042 &  & 0.486 & 0.153 & 0.048 & 0.015 \\
$8^{0.5}n^{0.125}$ &  & 1.339 & 0.431 & 0.140 & 0.045 &  & 0.487 & 0.156 & 0.051 & 0.017 \\
$2.5^{0.5}n^{0.25}$ &  & 1.337 & 0.444 & 0.148 & 0.050 &  & 0.486 & 0.161 & 0.055 & 0.020 \\
$0.05n$ &  & 1.337 & 0.542 & 0.292 & 0.213 &  & 0.486 & 0.228 & 0.184 & 0.179 \\
$n$ &  & 2.037 & 1.302 & 1.091 & 1.028 &  & 1.088 & 1.010 & 1.001 & 1.000 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel B: Complete randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.440 & 0.139 & 0.044 & 0.014 &  & 0.440 & 0.139 & 0.044 & 0.014 \\
$5$ &  & 0.461 & 0.145 & 0.046 & 0.014 &  & 0.461 & 0.145 & 0.046 & 0.014 \\
$8^{0.5}n^{0.125}$ &  & 0.456 & 0.145 & 0.046 & 0.015 &  & 0.456 & 0.145 & 0.046 & 0.015 \\
$2.5^{0.5}n^{0.25}$ &  & 0.461 & 0.145 & 0.046 & 0.015 &  & 0.461 & 0.145 & 0.046 & 0.015 \\
$0.05n$ &  & 0.461 & 0.146 & 0.046 & 0.015 &  & 0.461 & 0.146 & 0.046 & 0.015 \\
$n$ &  & 0.440 & 0.139 & 0.044 & 0.014 &  & 0.440 & 0.139 & 0.044 & 0.014 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel C: Paired randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.404 & 0.127 & 0.040 & 0.013 &  & 0.404 & 0.127 & 0.040 & 0.013 \\
$5$ &  & 0.424 & 0.134 & 0.042 & 0.013 &  & 0.424 & 0.134 & 0.042 & 0.013 \\
$8^{0.5}n^{0.125}$ &  & 0.422 & 0.134 & 0.042 & 0.013 &  & 0.422 & 0.134 & 0.042 & 0.013 \\
$2.5^{0.5}n^{0.25}$ &  & 0.424 & 0.134 & 0.042 & 0.014 &  & 0.424 & 0.134 & 0.042 & 0.014 \\
$0.05n$ &  & 0.424 & 0.134 & 0.043 & 0.014 &  & 0.424 & 0.134 & 0.043 & 0.014 \\
$n$ &  & 0.404 & 0.127 & 0.040 & 0.013 &  & 0.404 & 0.127 & 0.040 & 0.013 \\
\bottomrule \multicolumn{11}{l}{\footnotesize Note: Each cell presents the result from 50,000 draws from the data generating process.} \\
\end{tabular}


==> tab-randomweights-bias.tex <==
\begin{tabular}{l p{0.1in} rrrr p{0.15in} rrrr}
\multicolumn{11}{l}{Panel A: Bernoulli randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.006 & 0.005 & 0.000 & 0.000 &  & 0.002 & 0.000 & 0.000 & 0.000 \\
$5$ &  & 0.001 & 0.000 & 0.000 & 0.000 &  & 0.011 & 0.002 & 0.000 & 0.000 \\
$8^{0.5}n^{0.125}$ &  & 0.004 & 0.001 & 0.000 & 0.000 &  & 0.012 & 0.001 & 0.000 & 0.000 \\
$2.5^{0.5}n^{0.25}$ &  & 0.001 & 0.000 & 0.000 & 0.000 &  & 0.011 & 0.002 & 0.000 & 0.000 \\
$0.05n$ &  & 0.001 & 0.000 & 0.000 & 0.002 &  & 0.011 & 0.003 & 0.002 & 0.001 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel B: Complete randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.003 & 0.000 & 0.000 & 0.000 &  & 0.003 & 0.000 & 0.000 & 0.000 \\
$5$ &  & 0.012 & 0.002 & 0.000 & 0.000 &  & 0.012 & 0.002 & 0.000 & 0.000 \\
$8^{0.5}n^{0.125}$ &  & 0.014 & 0.001 & 0.001 & 0.000 &  & 0.014 & 0.001 & 0.001 & 0.000 \\
$2.5^{0.5}n^{0.25}$ &  & 0.012 & 0.001 & 0.000 & 0.000 &  & 0.012 & 0.001 & 0.000 & 0.000 \\
$0.05n$ &  & 0.012 & 0.002 & 0.001 & 0.001 &  & 0.012 & 0.002 & 0.001 & 0.001 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel C: Paired randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.001 & 0.000 & 0.000 & 0.000 &  & 0.001 & 0.000 & 0.000 & 0.000 \\
$5$ &  & 0.013 & 0.002 & 0.000 & 0.000 &  & 0.013 & 0.002 & 0.000 & 0.000 \\
$8^{0.5}n^{0.125}$ &  & 0.016 & 0.002 & 0.000 & 0.000 &  & 0.016 & 0.002 & 0.000 & 0.000 \\
$2.5^{0.5}n^{0.25}$ &  & 0.013 & 0.003 & 0.000 & 0.000 &  & 0.013 & 0.003 & 0.000 & 0.000 \\
$0.05n$ &  & 0.013 & 0.004 & 0.001 & 0.001 &  & 0.013 & 0.004 & 0.001 & 0.001 \\
\bottomrule \multicolumn{11}{l}{\footnotesize Note: Each cell presents the result from 50,000 draws from the data generating process.} \\
\end{tabular}


==> tab-randomweights-sd.tex <==
\begin{tabular}{l p{0.1in} rrrr p{0.15in} rrrr}
\multicolumn{11}{l}{Panel A: Bernoulli randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 1.181 & 0.375 & 0.119 & 0.037 &  & 0.444 & 0.139 & 0.044 & 0.014 \\
$5$ &  & 1.307 & 0.415 & 0.132 & 0.041 &  & 0.489 & 0.155 & 0.049 & 0.015 \\
$8^{0.5}n^{0.125}$ &  & 1.309 & 0.420 & 0.135 & 0.044 &  & 0.488 & 0.157 & 0.051 & 0.017 \\
$2.5^{0.5}n^{0.25}$ &  & 1.307 & 0.426 & 0.141 & 0.047 &  & 0.489 & 0.161 & 0.055 & 0.019 \\
$0.05n$ &  & 1.307 & 0.502 & 0.263 & 0.201 &  & 0.489 & 0.227 & 0.183 & 0.178 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel B: Complete randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.440 & 0.139 & 0.044 & 0.014 &  & 0.440 & 0.139 & 0.044 & 0.014 \\
$5$ &  & 0.469 & 0.149 & 0.047 & 0.015 &  & 0.469 & 0.149 & 0.047 & 0.015 \\
$8^{0.5}n^{0.125}$ &  & 0.467 & 0.150 & 0.048 & 0.016 &  & 0.467 & 0.150 & 0.048 & 0.016 \\
$2.5^{0.5}n^{0.25}$ &  & 0.469 & 0.153 & 0.051 & 0.018 &  & 0.469 & 0.153 & 0.051 & 0.018 \\
$0.05n$ &  & 0.469 & 0.197 & 0.149 & 0.144 &  & 0.469 & 0.197 & 0.149 & 0.144 \\
\bottomrule \\[\panelsep]
\multicolumn{11}{l}{Panel C: Paired randomization design} \\ \toprule
& & \multicolumn{4}{c}{Horvitz-Thompson estimator} & & \multicolumn{4}{c}{H\'ajek estimator} \\ \cmidrule{3-6} \cmidrule{8-11}
$a_n$ & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} & & \multicolumn{1}{l}{$n=10^2$} & \multicolumn{1}{l}{$n=10^3$} & \multicolumn{1}{l}{$n=10^4$} & \multicolumn{1}{l}{$n=10^5$} \\ \midrule
$1$ &  & 0.404 & 0.127 & 0.040 & 0.013 &  & 0.404 & 0.127 & 0.040 & 0.013 \\
$5$ &  & 0.438 & 0.138 & 0.044 & 0.014 &  & 0.438 & 0.138 & 0.044 & 0.014 \\
$8^{0.5}n^{0.125}$ &  & 0.435 & 0.140 & 0.045 & 0.015 &  & 0.435 & 0.140 & 0.045 & 0.015 \\
$2.5^{0.5}n^{0.25}$ &  & 0.438 & 0.143 & 0.048 & 0.017 &  & 0.438 & 0.143 & 0.048 & 0.017 \\
$0.05n$ &  & 0.438 & 0.191 & 0.148 & 0.143 &  & 0.438 & 0.191 & 0.148 & 0.143 \\
\bottomrule \multicolumn{11}{l}{\footnotesize Note: Each cell presents the result from 50,000 draws from the data generating process.} \\
\end{tabular}

